The Price of Differential Privacy for Low-Rank Factorization

In this paper, we study what price one has to pay to release {\em differentially private low-rank factorization} of a matrix. We consider various settings that are close to the real world applications of low-rank factorization: (i) the manner in which matrices are updated (row by row or in an arbitrary manner), (ii) whether matrices are distributed or not, and (iii) how the output is produced (once at the end of all updates, also known as {\em one-shot algorithms} or continually). Even though these settings are well studied without privacy, surprisingly, there are no private algorithm for these settings (except when a matrix is updated row by row). We present the first set of differentially private algorithms for all these settings. Our algorithms when private matrix is updated in an arbitrary manner promise differential privacy with respect to two stronger privacy guarantees than previously studied, use space and time {\em comparable} to the non-private algorithm, and achieve {\em optimal accuracy}. To complement our positive results, we also prove that the space required by our algorithms is optimal up to logarithmic factors. When data matrices are distributed over multiple servers, we give a non-interactive differentially private algorithm with communication cost independent of dimension. In concise, we give algorithms that incur optimal cost. We also perform experiments to verify that all our algorithms perform well in practice and outperform the best known algorithms until now for large range of parameters. We give experimental results for total approximation error and additive error for varying dimensions, $\alpha$ and $k$.

==> comparison.tex <==
\begin{table} [t!]
{
\small{
 \begin{center}
\begin{tabular}{|c|c|cc|}
\hline
	  				&					& Neighbouring Data  								  & Approximation (Multiplicative/Additive)
  \\ 
  					&  & Assumptions &  \\ \hline
\multirow{4}{*} {Problem~\ref{prob:private_factor}} 
&\multirow{1}{*}{\thmref{naive}}						& $\| \bA - {\bA}'\|_F = 1$	  & $\alpha$ \\% \cline{2-5}
& $(\varepsilon,\delta)$-differential privacy  & No assumptions & $\gamma=  O_\delta \paren{\frac{1}{\varepsilon} \paren{ \sqrt{(1+\alpha)km} + \sqrt{\frac{n}{\alpha}\max \set{k , \frac{1}{\alpha}} } }    }$ 
%\multicolumn{2}{l |}{$\qquad \alpha, \qquad \tau={O}\paren{\paren{ \sqrt{km} + \sqrt{\frac{n(1+\alpha)}{\alpha^3}\paren{k + \frac{1}{\alpha}} } }  \frac{\sqrt{\log(1/\delta)}}{\varepsilon}  }$}
\\ \cline{2-4}

%\multirow{4}{*} {Problem~\ref{prob:private_factor}} 
&\multirow{1}{*}{\thmref{low_space_private}}						& $\bA - {\bA}' =\mathbf{u} \mathbf{v}^{\mathsf T}$	  & $\alpha$ \\% \cline{2-5}
& $(\varepsilon,\delta)$-differential privacy  & No assumptions & $\gamma= O_\delta \paren{ \frac{1}{\varepsilon} \sqrt{\frac{1+\alpha}{1-\alpha}} \paren{ \sqrt{\frac{m}{\alpha}\max \set{k , \frac{1}{\alpha}}} + \sqrt{kn}} } $
%\multicolumn{2}{l |}{$\qquad \alpha, \qquad \tau=O\paren{   \frac{ \sqrt{(1+\alpha)k(m+n)\log(1/\delta)}}{\alpha \varepsilon}  } $}

\\ \hline

\multirow{4}{*} {Problem~\ref{prob:private_frob}} 
&\multirow{1}{*}{Hardt and Roth~\cite{HR12} }				& $\bA - {\bA}' = \mathbf{e}_s \mathbf{v}^{\mathsf T}$	& $O(1)$	 	 	 \\ %\cline{2-5}
 & $(\varepsilon,\delta)$-differential privacy  & Incoherent matrix & $\tau =O_\delta \paren{ \frac{ \sqrt{km}}{\varepsilon} + k \sqrt{ \frac{\mu_0 \|\bA\|_F }{\varepsilon} \sqrt{\frac{n}{m}}} }$
%  \multicolumn{2}{l |}{ $\qquad \alpha=O(1),    }  
  \\ \cline{2-4}

 &\multirow{1}{*}{Hardt and Roth~\cite{HR12} }				& $\bA - {\bA}' = \mathbf{e}_s \mathbf{v}^{\mathsf T}$	& $O(1)$	 	 	 \\ %\cline{2-5}
 & $(\varepsilon,\delta)$-differential privacy & No coherence assumption & $\tau =O_\delta \paren{ \frac{ \sqrt{km} }{\varepsilon} + \frac{k \sqrt{n}}{\varepsilon}  }$ %$O\paren{\varepsilon^{-1} \sqrt{km} \log (k/\delta) +  \sqrt{\mu_0 \|\bA\|_F} k n^{1/4}m^{-1/4} \sqrt{\varepsilon^{-1}\log(k/\delta)} }$
 % \multicolumn{2}{l |}{ $\qquad \alpha=O(1),  }  
  \\ \cline{2-4}

 
&\multirow{1}{*}{Upadhyay~\cite{Upadhyay14}}						& $\bA - {\bA}' = \mathbf{e}_s \mathbf{v}^{\mathsf T}$	& $O(1)$ \\% \cline{2-5}
& $(\varepsilon,\delta)$-differential privacy  &  No assumptions & $\tau=O_\delta\paren{ \frac{ k^2 \sqrt{n+m}}{\varepsilon}  }$
% \multicolumn{2}{l |}{$\qquad \alpha=O(1), \qquad \tau=O\paren{ \frac{ k^2 \sqrt{n+m} \log (k/\delta)}{\varepsilon}  }$}
\\ \hline%\cline{2-4}

\multirow{4}{*} {Problem~\ref{prob:private_spectral}} 
&\multirow{1}{*}{Kapralov and Talwar~\cite{KT13}}  &	 $\| \bA \|_2 -  \|{\bA}' \|_2 = 1$ 		& $0$					 	 \\ %\cline{2-5}
 &$\varepsilon$-differential privacy & Singular-value separation & $\tau=c \lambda_1,~\text{where}~\lambda_1 = \Omega \paren{ \frac{nk^3}{\varepsilon c^6} }$
 %\multicolumn{2}{l |}{$\qquad \alpha=0, \qquad \tau=c \lambda_1,~\text{where}~\lambda_1 = \Omega \paren{ \frac{nk^3}{\varepsilon c^6} }$}
   \\ \cline{2-4}

&\multirow{1}{*}{Hardt and Price~\cite{HP14}}					& $\bA - {\bA}'=\mathbf{e}_s \mathbf{e}_t^{\mathsf T}$ & $0$		 \\ %\cline{2-5}
 & $(\varepsilon,\delta)$-differential privacy & Incoherent matrix & $\tau=O_\delta \paren{ \frac{k^2}{\varepsilon} \sqrt{\mu + k \log n } }$
 % \multicolumn{2}{l |}{$\qquad \alpha=0, \qquad \tau=O \paren{ \frac{k^2}{\varepsilon} \sqrt{(\mu + k \log n) \log (1/\delta)} }$}
  \\ \hline


\multirow{4}{*}{Problem~\ref{prob:private_DTTZ}}  
&\multirow{1}{*}{Dwork {\it et al.}~\cite{DTTZ14}}			& $\bA - {\bA}' = \mathbf{e}_s \mathbf{v}^{\mathsf T}$ 	& $0$	 \\ %\cline{2-5}
& $(\varepsilon,\delta)$-differential privacy & No assumptions & $\tau=O_\delta \paren{ \frac{k\sqrt{n} }{\varepsilon} }$
%\multicolumn{2}{l |}{$\qquad \alpha=0, \qquad \tau=O \paren{ \frac{k\sqrt{n} \log(1/\delta)}{\varepsilon} }$} 
 \\ \cline{2-4}
 
&\multirow{1}{*}{Jiang {\it et al.}~\cite{JXZ15}} 					& $\bA - {\bA}' = \mathbf{e}_s \mathbf{e}_t^{\mathsf T}$ 	& $0$		\\ %\cline{2-5}
 & $\varepsilon$-differential privacy & No assumptions  & $\tau=O\paren{ \frac{n  \log n}{\varepsilon}}$
 %\multicolumn{2}{l |}{$\qquad \alpha=0, \qquad \tau=O\paren{ \frac{n  \log n}{\varepsilon}}$}
 \\ \hline
\end{tabular}
\caption{Comparison of Models for Differentially-private $k$-Rank Approximation ($\beta=O(1)$, $\mathbf{u}$ and $\mathbf{v}$ are unit vectors, $\mathbf{e}_s$ is the $s$-th standard basis, and $\mu_0$ and $\mu$ are coherence of the private matrix).} \label{others}% of an $n \times d$ rank-$\mathsf{rk}(A)$ matrix A.  $\mu$ denotes the coherence of $\bA$, $\gamma=\paren{\sigma_k/\sigma_{k+1}}-1$.} 
\label{table}
 \end{center}
}}
\end{table}

==> local.tex <==
%!TEX root = low.tex

\section{Noninteractive Local Differentially Private $\lrf$ Under $\priv_2$} \label{app:local}

\begin{definition}
(Local Differentially Private Principal Component Analysis Problem). Given an $m \times n$ matrix $\bA$ distributed among $m$ users where each user holds a row of the matrix $\bA$, a rank parameter $k$, and an accuracy parameter $0 < \alpha < 1$, design an algorithm in the model of Definition 15 which, upon termination, outputs an orthonormal matrix $\bU$ such that
$$  { \| \bA - \bU \bU^{\mathsf T}\bA \|_F \leq (1+\alpha) \| \bA - [\bA]_k  \|_F +\gamma }$$ with probability at least $1-\beta$,  
 and the communication cost of the algorithm is as small as possible. Furthermore, the algorithm should satisfies $(\varepsilon,\delta)$-LDP. 
\end{definition}

  \begin{figure}[t!]
 \begin{center}
\fbox{
\begin{minipage}[l]{6in}
{
\begin{center} {\scshape Private-Local-$\lrf$} \end{center}
{\bf Initialization.} Let $\eta=\max\set{k,\alpha^{-1}}$, $t=O(\eta \alpha^{-1}  \log (k/\delta)), v=O(\eta \alpha^{-2} \log(k/\delta))$. Let  $\rho_1={\sqrt{(1+\alpha)\ln(1/\delta)}}/{\varepsilon},~\rho_2={(1+\alpha)\sqrt{\ln(1/\delta)}}/{\varepsilon}$. 
	 Sample $\bPhi \sim \cN(0,1)^{n \times t}$, $\bPsi \sim \cN(0,1)^{t \times m}$,  $\bS \sim \cN(0,1)^{v \times m}$,  and $\bT \sim \cN(0,1)^{n \times v}$. Make them public.


\medskip \noindent \textbf{User-$i$ computation.} On input the row $\bA_{i:}$, user-$i$ does the following:
\begin{CompactEnumerate}
	 \item Sample  $\bN_{1,i} \sim \cN(0,\rho_1^2)^{1 \times t}$, $\bN_{2,i} \sim \cN(0,\rho_2^2)^{t \times v}$ and $\bN_{3,i} \sim \cN(0,\rho_2^2)^{v \times v}$. %, $\bN_1 \sim \cN(0,\rho_2^2)^{v \times v}$, and $\bN_1 \sim \cN(0,\rho_2^2)^{v \times v}$. 	
%	 \item Set $\sigma_\mathsf{min}={16 \log(1/\delta) \sqrt{t (1+\alpha)(1-\alpha)^{-1} \ln(1/\delta)}}/{\varepsilon}$.
	\item Set $\widehat{\bA}_{i:} \in \R^{m \times n}$ such that every row other than row-$i$ is an all zero vector. 
	Compute $\bY_{i:} = {\bA}_{i:} \bPhi + \bN_{1,i}$, $\widetilde{\bY}_{i:} = \bPsi \widehat{\bA}_{i:} \bT + \bN_{2,i} $, and $\bZ_{i:} = \bS \widehat{\bA}_{i:} \bT + \bN_{3,i}.$
\end{CompactEnumerate}

\medskip \noindent \textbf{Server side computation.} Once the server receives the reports from all the users, it follows the following steps.
\begin{CompactEnumerate}
	\item Form $\bY$ whose row-$i$ is $\bY_{i:}$. Compute $\bZ = \sum \bZ_{i:}$  and $\widetilde \bY  = \sum \widetilde{\bY}_{i:}$.
%	Compute a matrix $\bU \in \R^{m \times t}$ whose columns are orthonormal basis  for the column space of $\bY$.
%	\item Compute a SVD of $\mathbf{S} \bY := \widetilde{\bU}_s \widetilde{\bSigma}_s \widetilde{\bV}_s^{\mathsf T} \in \R^{v \times t}$.
%and a SVD of $ \bV\mathbf{T}^{\mathsf T}:=\widetilde{\bU}_t \widetilde{\bSigma}_t \widetilde{\bV}_t^{\mathsf T} \in \R^{t \times v}.$ 
	\item  Compute $\widetilde \bX:=\argmin_{\mathsf{rk}(\bX)\leq k} \|\bS \bY   \bX  \widetilde \bY  - \bZ \|_F$. 
	Compute a SVD of $\widetilde \bX$. Let it is be $\bU' \bSigma' \bV'^{\mathsf T}$. 
	\item Output the orthonormal basis $\bU$ for the span of $\bY \bU'$. 
\end{CompactEnumerate}

}
\end{minipage}
} \caption{Non-interactive Local Differentially private $\lrf$ Under $\priv_1$} \label{fig:local_spacelow}
\end{center}
\end{figure}

\begin{comment}
\begin{proof}
We will use~\lemref{phi} to prove the theorem. Set $\bPhi= \bPsi$, $\mathbf{P}=[\bA]_k$, $\mathbf{Q}=\bA$. Then for $\widetilde{\bX}=\argmin_{\bX} \|\bPsi ([\bA]_k \bX - \bA) \|$, we have with probability $1-\delta$ over $\bPsi \sim \cD_R$,
  \begin{align*} \| [\bA]_k^{\mathsf T} \widetilde{\bX} - \bA^{\mathsf T} \|_F &\leq (1+\alpha) \min_{\bX} \| [\bA]_k^{\mathsf T} \bX - \bA^{\mathsf T} \|_F \\
  		&\leq (1+\alpha)  \| [\bA]_k^{\mathsf T} - \bA^{\mathsf T} \|_F %\leq (1+\alpha) \| \bA^{\mathsf T} - [\bA]_k^{\mathsf T} \|_F
  \end{align*}
 Here $\widetilde{\bX} = (\bPsi [\bA]_k)^\dagger \bPsi \bA$. 
 In other words,%Since Frobenius norm is preserved under transpose, we have 
 \begin{align}
  \| [\bA]_k (\bPsi [\bA]_k )^\dagger  \bPsi \bA  - \bA \|_F \leq (1+\alpha) \| \bA - [\bA]_k \|_F. \label{eq:phipsi2}
 \end{align}
 
We now use~\lemref{phi} on the following regression problem: 
  \[\min_\bX \| \bPhi^{\mathsf T} (\mathbf{W} \bX - \bB)  \| \quad \min_{\bX} \|  \mathbf{W} \bX - \bB \|_F, \quad \text{where}~\mathbf{W}^{\mathsf T} = (\bPsi [\bA]_k)^\dagger \bPsi \bA~\text{and}~\bB = \bA^{\mathsf T} + (\bN_1 \bPhi^\dagger)^{\mathsf T} .\]

  Let $\widehat{\bX} := (\bPhi^{\mathsf T} \mathbf{W})^\dagger (\bPhi^{\mathsf T}\bB) = \argmin_{\bX} \| \bPhi^{\mathsf T} (\mathbf{W} \bX - \bA) \|_F.$ Since $[\bA]_k$ has rank $k$,~\lemref{phi} and~\eqnref{phipsi2} gives with probability $1-\delta$ over $\bPsi \sim \cD_R$ %using ,  we have
  \begin{align*}
  	\| (\bN_1 \bPhi^\dagger + \bA) \bPhi (\mathbf{W}^{\mathsf T} \bPhi)^\dagger \mathbf{W}^{\mathsf T} - \bB^{\mathsf T}\|_F 	&\leq (1+\alpha)\min_\bX \| \bX^{\mathsf T} \mathbf{W}^{\mathsf T} - \bB^{\mathsf T} \|_F \\
	&\leq (1+\alpha)^2 \| [\bA]_k (\bPhi [\bA]_k)^\dagger \bPhi \bA - \bB^{\mathsf T} \|_F \\
	& \leq (1+\alpha)^2 \| [\bA]_k (\bPhi [\bA]_k)^\dagger \bPhi \bA - \bA \|_F +(1+\alpha)^2 \| \bN_1 \bPhi^\dagger \|_F. 
   \end{align*}

 {Substituting the value of $\widehat{\bX}^{\mathsf T} := (\bB^{\mathsf T} \bPhi) (\mathbf{W}^{\mathsf T} \bPhi)^\dagger $, with probability $1-2\delta$ over $\bPhi^{\mathsf T}, \bPsi \sim \cD_R$, we have}
  \begin{align}
  \| \bA \bPhi ((\bPsi [\bA]_k)^\dagger \bPsi \bA \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger \bPsi \bA - \bA \|_F  \leq (1+\alpha)^2 (\| \bA - [\bA]_k \|_F + 2\| \bN_1 \bPhi^\dagger \|_F) \label{eq:BWZ16last2}  + \|\bN_1 \bPhi (\mathbf{W}^{\mathsf T} \bPhi)^\dagger \mathbf{W} \|_F
  \end{align}
 
% Since $ ([\bA]_k \bPhi)^{\dagger} (\bPsi \bA \bPhi ([\bA]_k \bPhi)^{\dagger})^\dagger$ has rank at most $k$ and scaling the value of $\alpha$ by a constant, we have the result. 
Since $ ((\bPsi [\bA]_k)^\dagger \bPsi \bA \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger$ has rank at most $k$, this implies that  %completes the proof because $\bPhi ([\bA]_k \bPhi)^{\dagger})^\dagger \bPsi$ is a rank-$k$ matrix.
\begin{align}
 	 \min_{\mathsf{rk}(\bX)\leq k} \| \bA \bPhi \bX \bPsi \bA - \bA \|_F	\leq (1+\alpha)^2 (\| \bA - [\bA]_k \|_F + 2\| \bN_1 \bPhi^\dagger \|_F)  + \|\bN_1 \bPhi (\mathbf{W}^{\mathsf T} \bPhi)^\dagger \mathbf{W} \|_F.
\end{align}

Let $\bC= (\bPsi \bA + \bN_2 \bT^\dagger)$.
Then 
\begin{align}
 	 \min_{\mathsf{rk}(\bX)\leq k} \| \bA \bPhi \bX \bC - \bA \|_F &\leq \| \bA \bPhi ((\bPsi [\bA]_k)^\dagger \bPsi \bA \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger \bC - \bA \|_F \\
	 	&\leq \| \bA \bPhi ((\bPsi [\bA]_k)^\dagger \bPsi \bA \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger \bPsi \bA - \bA \|_F \\
		&\quad  + \| \bA \bPhi ((\bPsi [\bA]_k)^\dagger \bPsi \bA \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger  \bN_2 \bT^\dagger \|_F.
\end{align}

 and consider the following two regression problems:
\begin{align}
	\widetilde{\bX}:= \argmin_{\mathsf{rk}(\bX)\leq k} \|\bS (\bA \bPhi  \bX \bC - \bA)\bT \|_F \quad 		\widehat \bX := \argmin_{\mathsf{rk}(\bX)\leq k} \| \bA \bPhi  \bX \bC - \bA \|_F
\end{align}

	Set $p=k/\alpha$, $\mathbf{D}=\bU$ and $\mathbf{E}=\bB$ in the statement of~\lemref{S}. Let us restrict our attention to  rank $k$ matrices $\bX$. % and denote by $\widehat{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bU \bX -\mathbf{E} \|_F$ and $\widetilde{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bS(\bU \bX -\bB) \|_F$. 
	Then we have with probability $1-\delta$ over $\bS \sim \cD_A$, 
	\begin{align}  
		(1 + \alpha)  \min_{\bX, \mathsf{r}(\bX)=k} \| \bA \bPhi \bX \bC  -\bA \|_F& = \| \bA \bPhi \widehat{\bX}  \bC - \bA \|_F  \geq (1 + \alpha)^{1/2} \| (\bA \bPhi \widehat{\bX}  \bC - \bA )\bS \|_F\nonumber \\
			& \geq (1 + \alpha)^{1/2}  \min_{\bX, \mathsf{r}(\bX)} \| (\bA \bPhi {\bX}  \bC - \bA )\bS \|_F \nonumber \\
			& = (1 + \alpha)^{1/2}  \| (\bA \bPhi \widetilde{\bX}  \bC - \bA  )\bS \|_F \nonumber \\
			& \geq    \| (\bA \bPhi \widetilde{\bX} \bC - \bA  ) \|_F %		\min_{\bX, \mathsf{r}(\bX)\leq k}\|\bS( \bU {\bX} - \bA) \|_F &\leq \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bU \bX - \bA \|_F 
			.  \label{eq:S2}  
	\end{align}

\end{proof}



%Alternate Proof
\pagebreak
\end{comment}

\begin{theorem} \label{thm:local}
 	Let  $m, n \in \N$ and $\alpha,\varepsilon,\delta$ be the input parameters.  Let $k$ be the desired rank of the factorization,  $s=\max\{m,n\}$, and $\eta=\max \set{k,\alpha^{-1}}$. Given a private input matrix $\bA \in \R^{m \times n}$ distributed in a row-wise manner amongst $n$ users, the output ${\bU}$ of  the algorithm, {\scshape Private-Local-$\lrf$}, presented in~\figref{streaming_private}, is a $k$-rank factorization and 
	satisfies the following properties:
	\begin{enumerate}
	\item  {\scshape Private-Local-$\lrf$} is a non-interactive $(\varepsilon,\delta)$-local differentially private under $\priv_2$. \label{local_privacy}
	\item  With probability $9/10$ over the coins of {\scshape Private-Local-$\lrf$}, \label{local_utility}
	 \begin{align*}
	  & \| \bA - \bU \bU^{\mathsf T}\bA \|_F \leq (1+ O(\alpha)) \| \bA - [\bA]_k \|_F + {O}\paren{ v\sqrt{m\rho_2} + \sqrt{vtm  \rho_2 } } .
	  \end{align*} 
	\item The bits of communication used by {\scshape Private-Streaming-Frobenius-$\lrf$} is $O(v^2)$. \label{local_bits}
	\item The time required to compute the factorization is $O\paren{(\mathsf{nn}(\bA) + \frac{(m+n	 \alpha^{-2})  \eta^2  \log^2(k/\delta)}{\alpha^{2}} +\frac{ \eta^3  \log^3(k/\delta)}{\alpha^{s3}}}$. \label{local_time}
	\end{enumerate}
 \end{theorem}


\begin{proof}
The local privacy is easy to follow from the Gaussian mechanism and as in~\lemref{low_space_private}.

Let $\bN_1$ be a random Gaussian matrices whose row-$i$ is $\bN_{1,i}$. Let $\bN_2 = \sum \bN_{2,i}, \bN_3 = \sum \bN_{3,i}$.
We will use~\lemref{phi} to prove the theorem. Set $\bPhi= \bPsi^{\mathsf T}$, $\mathbf{P}=([\bA]_k \bT)^{\mathsf T}$, $\mathbf{Q}=\bA  +  \bPsi^\dagger\bN_2 \bT^\dagger$. Let $\bC= (\bPsi \bA  + \bN_2 \bT^\dagger )$.
Then for $\widetilde{\bX}=\argmin_{\bX} \|\bPsi^{\mathsf T} (\bT^{\mathsf T}[\bA]_k^{\mathsf T} \bX - (\bT^{\mathsf T}\bA^{\mathsf T} + \bN_2^{\mathsf T})) \|$, we have with probability $1-2\delta$ over $\bPsi \sim \cD_R$ and $\bT \sim \cD_A$,
  \begin{align*} 
  \| \bT^{\mathsf T} [\bA]_k^{\mathsf T} \widetilde{\bX} - (\bT^{\mathsf T}\bA^{\mathsf T} + ( \bPsi^\dagger\bN_2)^{\mathsf T}) \|_F &\leq (1+\alpha) \min_{\bX} \|\bT^{\mathsf T} [\bA]_k^{\mathsf T} \bX - (\bT^{\mathsf T} \bA^{\mathsf T} +  \bPsi^\dagger\bN_2) \|_F \\
  		&\leq (1+\alpha)^2  \| [\bA]_k - \bA\|_F + (1+\alpha)\|  \bPsi^\dagger\bN_2 \|_F %\leq (1+\alpha) \| \bA^{\mathsf T} - [\bA]_k^{\mathsf T} \|_F
  \end{align*}
  In other words,
    \begin{align*} 
  \| \bT^{\mathsf T} [\bA]_k^{\mathsf T} \widetilde{\bX} - \bT^{\mathsf T}\bA^{\mathsf T}  \|_F \leq (1+\alpha)^2  \| [\bA]_k - \bA\|_F + (2+\alpha)\|  \bPsi^\dagger\bN_2 \|_F %\leq (1+\alpha) \| \bA^{\mathsf T} - [\bA]_k^{\mathsf T} \|_F
  \end{align*}
Further, with probability $1-\delta$ over $\bT \sim \cD_A$%Since Frobenius norm is preserved under transpose, we have 
\[
  \| [\bA]_k \widetilde{\bX} - \bA  \|_F \leq (1+\alpha)  \| \bT^{\mathsf T} [\bA]_k^{\mathsf T} \widetilde{\bX} - \bT^{\mathsf T}\bA^{\mathsf T}  \|_F \leq (1+\alpha)^3  \| [\bA]_k - \bA\|_F + (1 + \alpha)(2+\alpha)\|  \bPsi^\dagger\bN_2 \|_F %\leq (1+\alpha) \| \bA^{\mathsf T} - [\bA]_k^{\mathsf T} \|_F
\]
  
  
 Here $\widetilde{\bX} = (\bPsi \bT^{\mathsf T}[\bA]_k^{\mathsf T})^\dagger (\bPsi \bA \bT + \bN_2) = (\bPsi [\bA]_k)^\dagger \bC \bT$. Let $\mathbf{W}^\mathsf T = \widetilde \bX$. 
 \begin{align}
  \| [\bA]_k (\bPsi [\bA]_k )^\dagger  \bC \bT  - \bA  \|_F \leq (1+\alpha)^3 \| \bA - [\bA]_k \|_F + (1 + \alpha)(2+\alpha) \| \bPsi^\dagger \bN_2 \|_F. \label{eq:phipsi2}
 \end{align}
 
We now use~\lemref{phi} on the following regression problem: 
  \[\min_\bX \| \bPhi^{\mathsf T} (\mathbf{W} \bX - \bB)  \| \quad \min_{\bX} \|  \mathbf{W} \bX - \bB \|_F, \quad \text{where}~\bB = \bA^{\mathsf T} + (\bN_1 \bPhi^\dagger)^{\mathsf T} .\]

  Let $\widehat{\bX} := (\bPhi^{\mathsf T} \mathbf{W})^\dagger (\bPhi^{\mathsf T}\bB) = \argmin_{\bX} \| \bPhi^{\mathsf T} (\mathbf{W} \bX - \bA) \|_F.$ Since $[\bA]_k$ has rank $k$,~\lemref{phi} and~\eqnref{phipsi2} gives with probability $1-\delta$ over $\bPsi \sim \cD_R$ %using ,  we have
  \begin{align*}
%  	\| (\bN_1 \bPhi^\dagger + \bA) \bPhi (\mathbf{W}^{\mathsf T} \bPhi)^\dagger \mathbf{W}^{\mathsf T} - \bB^{\mathsf T}\|_F 	&\leq (1+\alpha)\min_\bX \| \bX^{\mathsf T} \mathbf{W}^{\mathsf T} - \bB^{\mathsf T} \|_F \\
  	\| \widehat \bX^\mathsf T \mathbf{W}^{\mathsf T} - \bB^{\mathsf T}\|_F 	&\leq (1+\alpha)\min_\bX \| \bX^{\mathsf T} \mathbf{W}^{\mathsf T} - \bB^{\mathsf T} \|_F \\
	&\leq (1+\alpha) \| [\bA]_k (\bPsi [\bA]_k)^\dagger \bC \bT - \bB^{\mathsf T} \|_F \\
	& \leq (1+\alpha) \| [\bA]_k (\bPsi [\bA]_k)^\dagger \bC \bT - \bA  \|_F +(1+\alpha) \| \bN_1 \bPhi^\dagger \|_F \\
	&\leq (1+\alpha)^4 \| \bA - [\bA]_k \|_F + (1 + \alpha)^2(2+\alpha) \| \bPsi^\dagger \bN_2 \|_F +(1+\alpha) \| \bN_1 \bPhi^\dagger \|_F.
   \end{align*}

In other words,
\[ \| \widehat \bX^\mathsf T \mathbf{W}^{\mathsf T} - \bA\|_F \leq (1+\alpha)^4 \| \bA - [\bA]_k \|_F + (1 + \alpha)^2(2+\alpha) \| \bPsi^\dagger \bN_2 \|_F +(2+\alpha) \| \bN_1 \bPhi^\dagger \|_F . \]
 {Substituting the value of $\widehat{\bX}^{\mathsf T} := (\bB^{\mathsf T} \bPhi) (\mathbf{W}^{\mathsf T} \bPhi)^\dagger  = (\bA \bPhi + \bN_1)  (\mathbf{W}^{\mathsf T} \bPhi)^\dagger = \bY  (\mathbf{W}^{\mathsf T} \bPhi)^\dagger$, with probability $1-2\delta$ over $\bPhi^{\mathsf T}, \bPsi \sim \cD_R$, we have}
  \begin{align*}
  \|  \bY  (\mathbf{W}^{\mathsf T} \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger  \bC \bT - \bA \|_F \leq (1+\alpha)^4 \| \bA - [\bA]_k \|_F + (1 + \alpha)^2(2+\alpha) \| \bPsi^\dagger \bN_2 \|_F +(2+\alpha) \| \bN_1 \bPhi^\dagger \|_F.  %+ \|\bN_1 \bPhi (\mathbf{W}^{\mathsf T} \bPhi)^\dagger \mathbf{W} \|_F
  \end{align*}
 
% Since $ ([\bA]_k \bPhi)^{\dagger} (\bPsi \bA \bPhi ([\bA]_k \bPhi)^{\dagger})^\dagger$ has rank at most $k$ and scaling the value of $\alpha$ by a constant, we have the result. 
Let $\mathbf{E} =\bA  + \bS^\dagger \bN_3 \bT^\dagger$. Since $ \bX_*:=  (\mathbf{W}^{\mathsf T} \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger$ has rank at most $k$, this implies that  %completes the proof because $\bPhi ([\bA]_k \bPhi)^{\dagger})^\dagger \bPsi$ is a rank-$k$ matrix.
\begin{align}
 	 \min_{\mathsf{rk}(\bX)\leq k} \| (\bY \bX  \bC \bT - \mathbf{E}) \|_F & \leq  \| (\bY \bX_* \bC \bT - \mathbf{E}) \|_F \\
	 &  \leq  \| (\bY \bX_* \bC \bT - \bA) \|_F  +  \|  \bS^\dagger \bN_3 \bT^\dagger  \|_F \nonumber \\
	 &\leq (1+\alpha)^4 \| \bA - [\bA]_k \|_F + (1 + \alpha)^2(2+\alpha) \| \bPsi^\dagger \bN_2 \|_F  \nonumber \\
	 &\qquad +(2+\alpha) \| \bN_1 \bPhi^\dagger \|_F +  (1+\alpha) \|  \bS^\dagger \bN_3 \bT^\dagger  \|_F.
\end{align}

%Then 
%\begin{align}
% 	 & \min_{\mathsf{rk}(\bX)\leq k} \| \bY \bX \bC - (\bA\bT + \bS^\dagger \bN_3) \|_F \leq  \| \bY \bX_* \bC - (\bA\bT + \bS^\dagger \bN_3) \|_F \nonumber
%	 \\ &\quad \leq(1+\alpha)^2 (\| \bA - [\bA]_k \|_F + 2\| \bN_1 \bPhi^\dagger \|_F)  + (1+\alpha)\|\bN_2\bT^\dagger \|_F + \|\bS^\dagger \bN_3) \|_F \nonumber 
%	 	&\leq (1+\alpha)^2 (\| \bA - [\bA]_k \|_F + 2\| \bN_1 \bPhi^\dagger \|_F)  + (1+\alpha)\|\bN_2\bT^\dagger \|_F \\
%		&\quad  + \| \bA \bPhi ((\bPsi [\bA]_k)^\dagger \bPsi \bA \bPhi)^\dagger (\bPsi [\bA]_k)^\dagger  \bN_2 \bT^\dagger \|_F + \| \bS^\dagger \bN_3) \|_F.
%\end{align}

Now consider the following two regression problems:
\begin{align}
	\widetilde{\bX}:= \argmin_{\mathsf{rk}(\bX)\leq k} \|\bS \bY   \bX \bC \bT  - \bS \mathbf{E} \|_F \quad 		\widehat \bX := \argmin_{\mathsf{rk}(\bX)\leq k} \| \bY  \bX \bC \bT  - \mathbf{E} \|_F
\end{align}

	Set $p=k/\alpha$, $\mathbf{D}=\bY   \bX \bC $ and $\mathbf{E}=\bA + \bS^\dagger \bN_3 \bT^\dagger$ in the statement of~\lemref{S}. Let us restrict our attention to  rank $k$ matrices $\bX$. % and denote by $\widehat{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bU \bX -\mathbf{E} \|_F$ and $\widetilde{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bS(\bU \bX -\bB) \|_F$. 
	Then we have with probability $1-\delta$ over $\bS \sim \cD_A$, 
	\begin{align}  
		 \min_{\bX, \mathsf{r}(\bX)=k} \| \bY \bX \bC \bT   - \mathbf{E}  \|_F^2 
		 &= \min_{\bX, \mathsf{r}(\bX)=k} \| \bY \bX \bC \bT   - (\bA + \bS^\dagger \bN_3 \bT^\dagger)  \|_F^2 \nonumber \\
		 & = \| \bY\widehat{\bX}  \bC \bT - (\bA + \bS^\dagger \bN_3 \bT^\dagger) \|_F^2 \nonumber \\
		 &  \geq (1 + \alpha) \| \bS(\bY \widehat{\bX}  \bC \bT  - (\bA + \bS^\dagger \bN_3 \bT^\dagger))  \|_F^2 \nonumber \\
			& \geq (1 + \alpha)  \min_{\bX, \mathsf{r}(\bX)} \|\bS (\bY {\bX}  \bC  - (\bA + \bS^\dagger \bN_3\bT^\dagger) ) \|_F \nonumber \\
%			&= (1 + \alpha)^{1/2}  \min_{\bX, \mathsf{r}(\bX)} \|\bS \bY {\bX}  (\bPsi \bA \bT + \bN_2) - (\bS \bA\bT + \bN_3) ) \|_F \nonumber \\
			&= (1 + \alpha) \| \bY \widetilde{\bX}  \bC - ( \bA + \bS^\dagger\bN_3 \bT^\dagger) ) \|_F \nonumber \\
			&\geq (1 + \alpha) \| \bY \widetilde{\bX}  \bC -  \bA \|_F  - (1+\alpha)\| \bS^\dagger\bN_3 \bT^\dagger) ) \|_F\nonumber
%			& = (1 + \alpha)^{1/2}  \| (\bY \widetilde{\bX}  \bC - \bA  )\bT \|_F \nonumber \\
%			& \geq    \| (\bY \widetilde{\bX} \bC \bT - (\bA \bT + \bN_3)  ) \|_F  \\%		\min_{\bX, \mathsf{r}(\bX)\leq k}\|\bS( \bU {\bX} - \bA) \|_F &\leq \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bU \bX - \bA \|_F 
%			& \geq (1+\alpha) \| (\bY \widetilde{\bX} (\bPsi \bA \bT + \bN_2) - (\bA \bT + \bN_3)  ) \|_F.  \label{eq:S2}  
	\end{align}
This completes the proof because $\bU \bU^{\mathsf T}$ projects the column of $\bA$ into the column space of $\bS \bY \widetilde \bX$.
\end{proof}

The following claim follows from~\lemref{SRHTinverse}.
\begin{claim} \label{claim:SRHTinversetwicelocal}
Let $\bS, \bT \sim \cD_A$. Then for any matrix $\bN_3$ of appropriate dimension,
 $ \|  \bS^\dagger \bN_3 (\bT^{\mathsf T})^\dagger \|_F = \| \bN_3 \|_F.$
\end{claim}

  \begin{lemma} \label{lem:noiselocal} \label{lem:naiveN_2}
 Let $\bN_1 \sim \cN(0,\rho^2)^{m \times t}$. Then  $\|  \bN_1 \bPhi^\dagger \|_F = O( \rho \sqrt{tn})$ with probability $99/100$ over $\bS \sim \cD_A$. 
 \end{lemma}
 \begin{proof} Using~\lemref{N}, we have $\E[ \| \bN_1 \|_F^2] = mt \rho^2.$ The result follows by invoking~\lemref{SRHTinverse} %(or~\lemref{efficiency})
  and Markov's inequality.
 \end{proof}

The following follows from Markov's inequality and that every entry of $\bN_2$ is distributed as $\cN(0,n)$.
\begin{claim} \label{claim:N_2local}
 $\|\bN_2 \|_F = O(nv^2)$ with probability $99/100$
\end{claim}






==> section3.tex <==
%!TEX root = low.tex

%\begin{extended}
%\begin{full}
%\section{Proof of~\thmref{space}} \label{app:space}
\section{Non-Private Space-Optimal Low-rank Factorization} \label{app:nonprivate}
The main focus of this paper is differentially private low-rank factorization. However, our observation about the algorithm of Boutsidis {\it et al.} also raises the natural  question about robust storage. The folklore approach in the literature of (non-private) streaming model of computation is to use error-correcting codes. However, such approach works when part of the storage is deleted or corrupted, but does not work when the storage incurs some additive noise.  In the standard theory of error-correcting codes, there is a rich literature of algebraic manipulation codes~\cite{CDFP08} which correct errors in the case of additive error, but they only work in finite fields. 
As we mentioned earlier, the naive approach to convert the algorithm of Boutsidis {\it et al.}~\cite{BWZ16} to a differentially private algorithm leads to a large additive error. In other words, it shows that noisy storage can lead to a large accuracy loss. This observation leads to the following question: %One can therefore ask the following question:
\begin{quote}
 {\bf Question 5.} Is it possible to achieve meaningful accuracy even when the storage is noisy?
\end{quote}

The algorithm of Boutsidis {\it et al.}~\cite{BWZ16} can be modified slightly to output a low-rank factorization. However, the output is still not a singular value decomposition, but a different form of low-rank factorization, i.e., one need to do extra computation to get the left and right singular vectors from the factorization they output (see~\appref{BWZ16} for more details). 
%As a corollary to~\thmref{low_space_private}, we get a space-optimal non-private algorithm for low-rank singular value decomposition by letting $\varepsilon \rightarrow \infty$. Our algorithm is  different from Boutsidis {\it et al.}~\cite{BWZ16} and answers question 5 mentioned earlier. %We use  {\em three} sketches to approximate the row-space, the column-space and the singular values of the matrix. 
%it makes our algorithm robust against noisy sketches in the sense that  (and not linearly as incurred by the algorithm of Boutsidis {\it et al.}~\cite{BWZ16}) for the same amount of noise.  %Even if one does count the update-time efficiency, we believe these factors makes our algorithm more reliable in the actual implementation. %We present our algorithm in~\secref{space}.
%The idea used behind the algorithm is that $\bY_c=  \bA\bPhi$ approximates the column-space, $\bY_r = \bPsi\bA $ approximates the row-space of the matrix $\bA$, and $\bZ = \bS \bA \bT^{\mathsf T}$ stores a sketch of the matrix $\bA$. 
%We show the following. %The term $\bZ = \bS \bA \bT^{\mathsf T}$ can be seen as approximating the . 
%We show the following
%\begin{quote}



 % \medskip \noindent \textbf{Optimality of the result.} 

%\medskip \noindent \textbf{Comparison of Non-private Algorithms.}
%Our non-private algorithm has a nice symmetric form. It uses basic linear algebra making it arguably simpler to state and analyze than the only known space-optimal algorithm of Boutsidis {\it et al.}~\cite{BWZ16}. 
% on 

One of the benefits of studying private algorithm is that, if we set $\varepsilon \rightarrow \infty$, then we get  a non-private algorithm. As a result, we have a direct corollary to~\thmref{low_space_private}. 
In our particular case, we can further improve the running time as we do not need the Gaussian matrix, $\Omega$. Instead we can sample $\Phi \sim \R^{m \times u}.$ 
We have the following result:



 \begin{figure}[t]
\begin{center}
 \fbox{
\begin{minipage}[l]{6in}
{
\begin{center} \underline{\scshape Optimal-Space-$\lrf$} \end{center}
\paragraph{Initialization.} Set $t=O(k\alpha^{-1}  \log(k/\delta)), v=O( k\alpha^{-2}  \log(k/\delta))$. Sample $\bPhi \in \R^{n \times t}, \bPsi  \in \R^{t \times m}$ such that $\bPhi^{\mathsf T} ,\bPsi \sim \cD_R$ satisfies~\lemref{phi}. Sample $\bS\in \R^{v \times m}, \bT \in \R^{v \times n}$ such that $\bS, \bT \sim \cD_A$  satisfies~\lemref{S}. Initialize  all zero matrices, $\bY_c:= \mathbf{0}^{m \times t},\bY_r:= \mathbf{0}^{t \times n}$, and $\bZ := \mathbf{0}^{v \times v}$. % Pick $\bPhi \in \R^{n \times k/\alpha}, \bPsi  \in \R^{k/\alpha \times m}$ as in~\lemref{CW13}, and $\bS\in \R^{k/\alpha^3 \times m}, \bT \in \R^{k/\alpha^3 \times n}$  such that  $\bS$ and $\bT$ are $(\alpha,\beta)$-affine embedding.
%	\item Compute $\bY_c= \bA \bPhi, $  $\bY_r=  \bPsi \bA,$ and $\bZ=\bS \bA \bT^{\mathsf T}$ in a single pass.

\medskip
%\paragraph{Update rule.}  Suppose at time $\tau$, the stream is $(i_\tau,j_\tau,\bA_{\tau})$, where $(i_\tau,j_\tau) \in [m] \times [n]$. Update the matrices by the following rule: (i) $(\bY_c)_{i_\tau,j} = (\bY_c)_{i_\tau,j} + \bA_\tau \bPhi_{j_\tau,j}$ for all $1 \leq j \leq t$, (ii) $(\bY_r)_{i,j_\tau} = (\bY_c)_{i,j_\tau} + \bA_\tau \bPsi_{i,j_\tau}$ for all $1 \leq j \leq t$, and (iii) $\bZ_{i,j}= \bZ_{i,j} + \bS_{i,i_\tau} \bA_\tau \bT_{j,j_\tau}$ for all $1 \leq i,j \leq v$.

\paragraph{Update rule.}  Suppose at time $\tau$, the stream is $(i_\tau,j_\tau,\Delta_{\tau})$, where $(i_\tau,j_\tau) \in [m] \times [n]$ and $\Delta_\tau \in \R$. Let $\bA_\tau$ be a matrix with only non-zero entry $\Delta_\tau$ in position $(i_\tau,j_\tau)$. Update the matrices by the following rule: (i) $\bY_c = \bY_c + \bA_\tau \bPhi$, (ii) $\bY_r = \bY_r +   \bPsi \bA_\tau $, and (iii) $\bZ= \bZ + \bS \bA_\tau \bT^{\mathsf T}$.


\medskip
\paragraph{Computing the factorization.} %Return the output of  {\scshape Factor}$(\bY_c,\bY_r,\bZ,\bS,\bT,m,n,k,t,v)$.
Follow the following steps:
%\medskip
%\paragraph{ {\scshape Factor}$(\bY_c,\bY_r,\bZ,\bS,\bT,m,n,k,t,v)$}
\begin{enumerate}
	\item Compute a matrix $\bU \in \R^{m \times t}$ whose columns are orthonormal basis  for the column space of $\bY_c$ and matrix $\bV \in \R^{t \times n}$ whose rows are the orthonormal basis for the row space of $\bY_r$.
	\item Compute a SVD of $\mathbf{S} \bU := \widetilde{\bU}_s \widetilde{\bSigma}_s \widetilde{\bV}_s^{\mathsf T} \in \R^{v \times t}$ 
and a SVD of $ \bV\mathbf{T}^{\mathsf T}:=\widetilde{\bU}_t \widetilde{\bSigma}_t \widetilde{\bV}_t^{\mathsf T} \in \R^{t \times v}.$ 
	\item Compute a SVD of $ \widetilde{\bV}_s \widetilde{\bSigma}_s^{\dagger} [\widetilde{\bU}_s^{\mathsf T} \mathbf{Z} \widetilde{\bV}_t]_k \widetilde{\bSigma}_t^{\dagger} \widetilde{\bU}_t^{\mathsf T} $. Let it is be $\bU' \bSigma' \bV'^{\mathsf T}$. 
	\item Output the matrix  $\widetilde{\bU}=\bU \bU'$ compromising of left singular vectors, diagonal matrix $\widetilde{\bSigma}=\bSigma'$, and the matrix $\widetilde{\bV}=\bV^{\mathsf T} \bV' $ with right-singular vectors. 
\end{enumerate}

}\end{minipage}
} \caption{Space-efficient Low-rank Factorization} \label{fig:spacelow}
\end{center}
\end{figure}

 \begin{theorem} \label{thm:space}
	Let $m,n \in \N$, $\alpha,\varepsilon, \delta$ be the input parameters, and $k$ be the desired rank of the low-rank factorization. Given a matrix $\bA \in \R^{m \times n}$ in the turnstile model, there is an algorithm that outputs a rank-$k$ factorization $\widetilde{\bU}, \widetilde{\bSigma}, \widetilde{\bV}$ 
	% (page~\pageref{fig:spacelow}), 
	 of the matrix $\bA$ such that:
	\begin{enumerate}
		\item With probability $9/10$ over the random coins of the algorithm {\scshape Optimal-Space-$\lrf$}, \label{correctness}
	 \begin{align*}
 %\| \bU \widetilde{\bV}_s \widetilde{\bSigma}_s^\dagger [\widetilde{\bU}_s^{\mathsf T} \bZ \widetilde{\bV}_t ]_k \widetilde{\bSigma}_t^\dagger \widetilde{\bU}_t^{\mathsf T} \bV^{\mathsf T} - \bA \|_F  \leq (1+\alpha) \|\bA - [\bA]_k\|_F .
 \| \mathbf{M}_k - \bA \|_F  \leq (1+\alpha) \|\bA - [\bA]_k\|_F,~\text{where}~ \mathbf{M}_k = \widetilde{\bU} \widetilde{\bSigma} \widetilde{\bV}^{\mathsf T}.
   \end{align*} %where $\bU,\bU',\bSigma',\bV,\bV'$ are as defined in~\figref{spacelow}.
		\item %The update-time of {\scshape Optimal-Space-$\lrf$}  is $O(k/\alpha^2 \log(k/\delta))$.  
		The total computational time of {\scshape Optimal-Space-$\lrf$} is $O(\mathsf{nn}(\bA) \log(1/\delta)+(m+n) k^2 \alpha^{-2} \log(k/\delta) +k^3/\alpha^5 \log^3(k/\delta) )$. \label{time}
		\item {\scshape Optimal-Space-$\lrf$} uses at most $O\paren{\frac{(m+n)k}{ \alpha} \log\paren{{k}} }$ space. \label{space}
   \end{enumerate}
\end{theorem}

 Before we give a proof of~\thmref{space}, we first state the direct implications of our result.~\thmref{space} shows that our algorithm uses optimal space due to the lower bound result of Clarkson and Woodruff~\cite{CW09}. 
  Our algorithm is  more robust with respect to noisy sketches than Boutsidis {\it et al.}~\cite{BWZ16} in the sense that,  for similarly distributed noise matrices, we incur an additive error   proportional to $\sqrt{m}$ and $\sqrt{n}$ while Boutsidis {\it et al.}~\cite{BWZ16} incurs  a large additive error (see~\appref{BWZ16}). Robustness with respect to noise is one of the desirable features in many applications from the point of view of both theory and practice. %Moreover, they 
\begin{comment}
\begin{table}[h]
\small{
 \begin{center}
\begin{tabular}{|c|c|c|}
\hline
  & Space & $\#$ sketches \\ \hline
 Clarkson-Woodruff~\cite{CW13} 
 %& ${O}(\mathsf{nn}(\bA) + mk^2/\alpha^2 + nk^{2}/\alpha^4)$ 
 & ${O}(mk/\alpha + nk/\alpha^2)$ & $2$\\ \hline
 Boutsidis {\it et al.}~\cite{BWZ16} 
 %& $O(\mathsf{nn}(\bA) + \poly(k/\alpha) + (m + n)k^2/\alpha)$ 
 & $O((n+m)k /\alpha)$ & $5$\\ \hline
 This work 
 %& ${O}(\mathsf{nn}(\bA) + (m+n)k^2/\alpha^2 + k^3 /\alpha^5)$ 
 & $O((n+m)k /\alpha)$ & $3$\\ \hline
 Lower Bound 
 %& $\Omega(\mathsf{nn}(\bA))$ 
 & $\Omega((n+m)k /\alpha)$~\cite{CW09} & $-$ \\ \hline
 \end{tabular}
 \caption{Comparison of  Non-private Algorithms for $(\alpha, 1/10, 0,k)\mbox{-}\mathsf{LRF}$} \label{table:nonprivate}
\end{center}
}
\end{table}
\end{comment}

We now return to the full proof of~\thmref{space}.
%\end{full}
\begin{proof}[Proof of~\thmref{space}]
Part~\ref{space} of~\thmref{space} follows straightforwardly from the choice of $v$ and $t$ and the dimensions of all  the sketches, $\bY_c = \bA \bPhi, \bY_r = \bPsi \bA$, and $\bZ = \bS \bA \bT^{\mathsf T}$. 
%For the update time in part~\ref{time} of~\thmref{space}, note that $\bPhi$ and $\bPsi$ operates in input-sparsity time, which is constant, plus an $O(\log(m+n))$ term. The same is true for the update time of $\bZ$. 
%For the update time, note that $\bPhi,\bPsi$ satisfies~\lemref{phi} and $\bS$ and $\bT$ satisfies~\lemref{S}. Since $\bA_\tau$ is all zero matrix except for $(i,j)$-entry, we only need to compute sketch of one column and one row in $\bA_\tau$, i.e.,  $\mathsf{nn}(\bA_\tau)=1$ and $n=1$ in~\lemref{phi} and~\lemref{S}. Therefore, computing $\bA_\tau \bPhi, \bPsi \bA_\tau,$ and $\bS \bA_\tau \bT^{\mathsf T}$ takes  $O(t \log t)$ time (for updating $\bY_c$ and $\bY_r$ and $O(v \log v)$ time (for updating $\bZ$). %Let . 

For the factorization time in part~\ref{time} of~\thmref{space}, we need to analyze the running time of the algorithm presented in~\figref{spacelow}. We analyze it as follows.
\begin{enumerate}
	 \item Computing $\bY_c$ requires $ O(\mathsf{nn}(\bA) \log (1/\delta))+ mt^2$ time and computing $\bY_r$ requires $O(\mathsf{nn}(\bA)\log (1/\delta)) + nt^2$ time. Therefore, computing $\bY_c$ and $\bY_r$ requires $ O(\mathsf{nn}(\bA) \log( k/\delta) +(m+n)k^2 \alpha^{-2} \log^2(k/\delta)$ time. Computing $\bZ$ requires $O(\mathsf{nn}(\bA) \log( 1/\delta)  +  k^2/\alpha^2 \log^2( k/\delta) + nk^2\alpha^{-2} \log^2( k/\delta))$
	 \item Computing the orthonormal basis $\bU$ and $\bV$ requires $nt^2 + mt^2 = O((m+n)k^2 \alpha^{-2} \log^2( k/\delta))$ time.
	 \item Computing a SVD of the matrix $\bS \bU$  and $\mathbf{T} \bV^{\mathsf T}$ requires $vt^2 + tv^2=O(k^3 \alpha^{-5} \log^2( k/\delta))$.
	 \item Computation of $[\widetilde{\bU}_s^{\mathsf T}\bZ \widetilde{\bV}]_k$ requires $O_\delta(\mathsf{nn}(\bA)) + tv^2= O(\mathsf{nn}(\bA) + k^{3} \alpha^{-5} \log^3 ( k/\delta))$ time.
	 \item Computation of the product $ \widetilde{\bV}_s \widetilde{\bSigma}_s^{\dagger} [\widetilde{\bU}_s^{\mathsf T} \mathbf{Z} \widetilde{\bV}_t]_k \widetilde{\bSigma}_t^{\dagger} \widetilde{\bU}_t^{\mathsf T} $ and its SVD  requires $(m+n)t^2=O((m+n) k^2 \alpha^{-2} \log^2( k/\delta))$ time.
\end{enumerate}

To prove part~\ref{correctness}, we use~\thmref{BWZ16}.~\thmref{BWZ16} relates $ \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bA \bPhi \bX \bPsi \bA  - \bA \|_F$ with $(1+\alpha)^2 \| \bA - [\bA]_k \|_F$ as follow.
\begin{align} \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bA \bPhi \bX \bPsi \bA  - \bA \|_F \leq (1+\alpha)^2 \| \bA - [\bA]_k \|_F. \label{eq:step14a} \end{align}
 
%We now lower bound $ \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bA \bPhi \bX \bPsi \bA  - \bA \|_F$ in terms of a basis for the column space of $\bA \bPhi$ and row space of $\bPsi \bA$. 
Since $\bV$ is a matrix whose rows are an orthonormal basis for the row space of $\bPsi \bA$  and $\bU$ is a matrix whose columns are an orthonormal basis for the column space of $\bA \bPhi$, we have
	\begin{align} 
		\min_{\bX, r(\bX) \leq k} \| \bU \bX \bV - \bA \|_F & \leq \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bA \bPhi \bX \bV - \bA \|_F \leq \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bA \bPhi \bX \bPsi \bA - \bA \|_F. \label{eq:basis4}  
	\end{align}
	Combining~\eqnref{step14a} and~\eqnref{basis4}, we have with probability $1-2\delta$ over $\bPhi, \bPsi \sim \cD_R$,  
	\begin{align} 
	\min_{\bY, r(\bY) \leq k} \| \bU \bX \bV - \bA \|_F \leq (1+\alpha)^2 \| \bA - [\bA]_k \|_F. \label{eq:step24}
	\end{align}
%	 In the next two steps, we show why the choice of $\bY=\widetilde{\bV}_s \widetilde{\bSigma}_s^\dagger [\widetilde{\bU}_s^{\mathsf T} \bS \bB \bT^{\mathsf T} \widetilde{\bV}_t ]_k \widetilde{\bSigma}_t^\dagger  \widetilde{\bU}_t^{\mathsf T}$ satisfies~\eqnref{basis4}.
%	\item [Step 2:]  
\begin{lemma} \label{lem:thirdspace}
Let $\bU$ and $\bV$ be as defined above and $\widetilde{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bS(\bU \bX \bV^{\mathsf T}  -\bA)\bT^{\mathsf T} \|_F$. Let $\cD_A$ be a distribution that satisfies  $(\alpha,\delta)$-subspace embedding. Then with probability $1-O(\delta)$ over $\bS,\bT^{\mathsf T} \sim \cD_A$,
\[	\|( \bU \widetilde{\bX} \bV  - \bA) \|_F \leq {(1+\alpha)^4} \| \bA - [\bA]_k \|_F. \]
\end{lemma}
\begin{proof}
Set $p=k/\alpha$, $\mathbf{D}=\bU$ and $\mathbf{E}=\bA$ in the statement of~\lemref{S} and $v=O(\eta/\alpha^2 \log (k/\alpha))$. Let us restrict our attention to only rank $k$ matrices $\bX$ and denote by $\widehat{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bU \bX\bV -\bA \|_F$ and $\widetilde{\bX}= \argmin_{\bX, \mathsf{r}(\bX)=k} \| \bS(\bU \bX \bV^{\mathsf T}  -\bA)\bT^{\mathsf T} \|_F$. Then, with probability $1-\delta$ over $\bS \sim \cD_A$, 
	\begin{align}  
		\min_{\bX, \mathsf{r}(\bX)=k} \| \bU \bX \bV -\bA \|_F &= \| \bU \widehat{\bX}  \bV - \bA \|_F \geq (1 + \alpha)^{-1/2} \| \bS(\bU \widehat{\bX}  \bV - \bA ) \|_F  \label{eq:34b} 
	\end{align}
		{Substituting $\mathbf{D}=\bV^{\mathsf T}$, $\bX = (\bS \bU \widehat{\bX})^{\mathsf T}$ and $\mathbf{E}=(\bS\bA)^{\mathsf T}$ in the statement of~\lemref{S}, with probability $1-O(\delta)$ over $\bS,\bT^{\mathsf T} \sim \cD_A$,}
	\begin{align}
		  (1 + \alpha)^{-1/2} \| \bS(\bU \widehat{\bX}  \bV - \bA ) \|_F  &  = (1 + \alpha)^{-1/2} \| \bV^{\mathsf T} (\bS\bU \widehat{\bX}) ^{\mathsf T} - (\bS\bA)^{\mathsf T} ) \|_F \nonumber \\
		 	& \geq (1 + \alpha)^{-1} \| \bT(\bV^{\mathsf T} (\bS\bU \widehat{\bX}) ^{\mathsf T} - (\bS\bA)^{\mathsf T} ) \|_F  \nonumber \\
		 	& = (1 +  \alpha)^{-1}  \| \bS(\bU \widehat{\bX}  \bV - \bA ) \bT^{\mathsf T}\|_F \nonumber \\
		 	& \geq (1 + \alpha)^{-1}  \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bS(\bU {\bX}  \bV - \bA ) \bT^{\mathsf T}\|_F   \nonumber \\
			& = (1 + \alpha)^{-1}  \| \bS(\bU \widetilde{\bX}  \bV - \bA  )  \bT^{\mathsf T} \|_F \nonumber \\ 
			& \geq (1 + \alpha)^{-3/2}  \| (\bU \widetilde{\bX}  \bV - \bA  )  \bT^{\mathsf T} \|_F   \nonumber \\
			& \geq   (1 + \alpha)^{-2} \| (\bU \widetilde{\bX}  \bV  - \bA  ) \|_F.  
%		\min_{\bX, \mathsf{r}(\bX)\leq k}\|\bS( \bU {\bX} - \bA) \|_F &\leq \min_{\bX, \mathsf{r}(\bX) \leq k} \| \bU \bX - \bA \|_F 
			\label{eq:S4}  
	\end{align}
	Combining~\eqnref{S4} with~\eqnref{step24} and~\eqnref{34b}, we have with probability $1-O(\delta)$ over the coins of {\scshape Optimal-Space}-$\lrf$, %$\bS,\bT \sim \cD_A$,  
	\begin{align}
	\|( \bU \widetilde{\bX} \bV  - \bA) \|_F \leq {(1+\alpha)^4} \| \bA - [\bA]_k \|_F. \label{eq:step34} 
	\end{align}
This completes the proof of~\lemref{thirdspace}.
\end{proof}

	To finalize the proof of~\thmref{space}, we need to compute $\widetilde{\bX}=\argmin_{\bX, \mathsf{r}(\bX) \leq k} \| \bS(\bU \bX \bV - \bA) \bT^{\mathsf T} \|_F$. If there were no rank constraints on the optimization problem, this is an easy problem. However, for solving the optimization problem under the rank constraint, we need~\lemref{orthonormal} to compute $\widetilde{\bX}$.  

	We now complete the proof of~\thmref{space}. Recall that $\bS \bU = \bU_s \bSigma_s \bV_s^{\mathsf T}$ and $\bT \bV^{\mathsf T} = \bU_t \bSigma_t \bV_t^{\mathsf T}$. Invoking~\lemref{orthonormal} with $\mathbf{C} = \widetilde{\bU}_s, \mathbf{R} = \widetilde{\bV}_t^{\mathsf T}$ and $\mathbf{F} = \bZ= \bS \bA \bT^{\mathsf T}$, we  get 
 \begin{align}
 [ \widetilde{\bU}_s^{\mathsf T} \bZ \widetilde{\bV}_t]_k &=  [ \widetilde{\bU}_s^{\mathsf T} \bS \bA \bT^{\mathsf T} \widetilde{\bV}_t]_k = \argmin_{\bX, \mathsf{r}(\bX) \leq k} \| \widetilde{\bU}_s \bX \widetilde{\bV}_t^{\mathsf T}- \bS \bA \bT^{\mathsf T} \|_F  \nonumber %\\ 
	 \end{align}
This implies that
 \begin{align}
  \widetilde{\bX} & =\widetilde{\bV}_s \widetilde{\bSigma}_s^\dagger [\widetilde{\bU}_s^{\mathsf T} \bZ \widetilde{\bV}_t ]_k \widetilde{\bSigma}_t^\dagger \widetilde{\bU}_t^{\mathsf T} 
= \argmin_{\bX, \mathsf{r}(\bX) \leq k} \| \bS(\bU \bX \bV - \bA) \bT^{\mathsf T} \|_F. \label{eq:solution4}
	 \end{align}
%\end{description}
Substituting~\eqnref{solution4} in~\eqnref{step34}, and adjusting the value of $\alpha$ by a constant, we have the final result.
% \[ \| \bU\widetilde{\bV}_s \widetilde{\bSigma}_s^\dagger [\widetilde{\bU}_s^{\mathsf T} \bZ \widetilde{\bV}_t ]_k \widetilde{\bSigma}_t^\dagger \widetilde{\bU}_t^{\mathsf T} \bV^{\mathsf T} - \bA \|_F \leq (1+\alpha) \|\bA - [\bA]_k\|_F. \]
\end{proof}
%\end{extended}


%We also need just three out of the five sketches of Boutsidis {\it et al.}~\cite{BWZ16}. % and one reason why we get an optimal error bound in the private setting. %Further, our algorithm shows that three sketches of Boutsidis {\it et al.}~\cite{BWZ16} are enough to get a low-rank factorization without a need to solve an optimization problem over the space of low-rank matrices.  %gave the first space-optimal algorithm for low-rank approximation; however, they run in time $O(mnk)$. This bound can be improved to achieved using the projection of Clarkson and Woodruff~\cite{CW13} as shown by Woodruff~\cite{Woodruff16}. %Moreover, their algorithm maintains five sketches. On the other hand, our algorithm achieves the same space bound and same approximation guarantee, runs in time linear in the dimension of the matrix and the input sparsity, and maintains just three sketches. We believe this makes our algorithm more practical. 
Our algorithm is more efficient in terms of both space and time than Clarkson and Woodruff~\cite{CW13} when $n >m/\alpha$. 
%Prior to our work, Boutsidis {\it et al.}~\cite{BWZ16} gave a space-optimal algorithm for $\lra$, but they do not optimize for run-time\footnote{After learning of an earlier draft of this paper~\cite{Upadhyay16}, in a personal communication, Woodruff~\cite{Woodruff16} showed that one can obtain the similar running time  as achieved by us%by using the embedding of Clarkson and Woodruff~\cite{CW13} in the algorithm of Boutsidis {\it et al.}~\cite{BWZ16}
%.}  and maintains five sketches. % We show that three of their sketches suffices for computing an $\lrf$.
We compare our results with previous results in Table~\ref{table:nonprivate}. 
